HyperDreamer: Hyper-Realistic 3D Content Generation and Editing from a Single Image

3D content creation from a single image is a long-standing yet highly desirable task. Recent advances introduce 2D diffusion priors, yielding reasonable results. However, existing methods are not hyper-realistic enough for post-generation usage, as users cannot view, render and edit the resulting 3D content from a full range. To address these challenges, we introduce HyperDreamer with several key designs and appealing properties: 1) Viewable: 360 degree mesh modeling with high-resolution textures enables the creation of visually compelling 3D models from a full range of observation points. 2) Renderable: Fine-grained semantic segmentation and data-driven priors are incorporated as guidance to learn reasonable albedo, roughness, and specular properties of the materials, enabling semantic-aware arbitrary material estimation. 3) Editable: For a generated model or their own data, users can interactively select any region via a few clicks and efficiently edit the texture with text-based guidance. Extensive experiments demonstrate the effectiveness of HyperDreamer in modeling region-aware materials with high-resolution textures and enabling user-friendly editing. We believe that HyperDreamer holds promise for advancing 3D content creation and finding applications in various domains.

==> articles/backup_texts.tex <==
%
\subsection{Appearance Modeling.}
\label{supp:appearance}
To enable a more realistic rendering, we introduce the Physically-Based Rendering (PBR) material model. Following TANGO~\cite{chen2022tango} and PhySG~\cite{physg2021}, we leverage spatially varying BRDF (SVBRDF) to parameterize the material, including roughness, specular, and normal.
% roughness $k_r \in \mathbbm{R}^2$, specular $k_s \in \mathbbm{R}^2$, and normal $k_n \in \mathbbm{R}^3$.
Based on the rendering equation~\cite{kajiya1986rendering}, given a location $x$ and the surface normal $n$, the incident light intensity at this point is denoted as $L_i(\omega_i;x)$ along the direction $\omega_i$; BRDF $f_r(\omega_o,\omega_i;x)$ denotes the reflectance coefficient of the material viewing from direction $\omega_o$. The observed light intensity $L_o(\omega_0;x)$ over the hemisphere $\Omega=\{\omega_i:\omega_i \cdot n > 0\}$ can be calculated as:

\begin{equation}
    L_o(\omega_0;x) = \int_\Omega L_i(\omega_i;x) f_r(\omega_o,\omega_i;x) (\omega_i \cdot n) d\omega_i .
    \label{eq:render_equation}
\end{equation}

We then utilize spherical Gaussians (SGs)~\cite{yan2012accurate} to approximate the rendering equation. For a sphere Gaussian with $n$ dimensions, given the lobe axis $\xi \in \mathbbm{S}^2$, the lobe sharpness $\lambda \in \mathbbm{R}_+$, and the lobe amplitude $\mu \in \mathbbm{R}^n_+$, the spherical function is formulated as:

\begin{equation}
    G(\nu;\xi,\lambda,\mu) = \mu e^{\lambda (\nu \cdot \xi - 1)},
    \label{eq:spherical_function}
\end{equation}
where $\nu \in \mathbbm{S}^2$ denotes the input.
The environment map $L(\omega_i)$ is represented with a mixture of $M$ SGs:

\begin{equation}
    L_i(\omega_i) = \sum\limits_{k=1}^{M} G(\omega_i;\xi_k,\lambda_k,\mu_k).
    \label{eq:environment_map}
\end{equation}

The SVBRDF function is composed of a diffuse albedo term $a_x = f_d(x)$ and a specular term $f_s(\omega_o,\omega_i,x)$. We adopt Instant-NGP~\cite{muller2022instant} as the appearance network, and $f_d(x)$ is modeled as an MLP based on the multi-resolution hash input encoding.  
We use the simplified Disney BRDF model~\cite{burley2012physically} for the specular term as $f_s(\omega_o,\omega_i) = \mathcal{M}(\omega_o,\omega_i)\mathcal{D}(h)$, where $h = (\omega_o + \omega_i)/||(\omega_o+\omega_i)||$ is the half vector, $\mathcal{M}$ is the Fresnel and shadowing effects, approximated by $\mathcal{M}_x \approx \mathcal{M}(\omega_o, 2(\omega_o \cdot n)n  \omega_o)$ following~\cite{physg2021}, and $\mathcal{D}$ is the normalized distribution function, which can be represented as a single SG. The specular term is thus formulated as:

\begin{equation}
    f_s(\omega_o,\omega_i;x) =  G(h;n_x,\frac{\lambda_x}{4h \cdot \omega_o},\mathcal{M}_x\mu_x),
    \label{eq:specular_tern}
\end{equation}
and we can obtain $f_r(\omega_o,\omega_i;x) = f_d(x)/\pi + f_s(\omega_o,\omega_i;x)$.
Finally, we follow~\cite{physg2021} to approximate the last term remained in Eqn.~\ref{eq:render_equation}, $\omega_i \cdot n$, by:
\begin{equation}
    \omega_i \cdot n = G(\omega_i;0.0315,n,32.7080) - 31.7003.
\end{equation}

The learnable parameters above include $\{\xi_k,\lambda_k,\mu_k\}_{k=1}^M$ for the environmental map, diffuse albedo $f_d$, and the spatially varying $\{\lambda, \mu\}$. 
Unlike TANGO which adopts two MLPs to predict $\{\lambda_x, \mu_x\}$ at location $x$, we assume that regions with the same semantic label usually share alike materials. Similar to the albedo learning, we maintain two semantic-aware learnable vectors for roughness $R_s$ and specular $S_s$. The dimensions of them are $N_s \times 1$ and $N_s \times 3$, respectively. We assume the specular color to be white, and thus the three channels in $R_s$ are forced the same. We also incorporate two MLP-based predictors to predict offsets for roughness and specular based on $R_s$ and $S_s$ to enable a more flexible and \needcheck{fine-grained} material modeling.

Finally, we use an off-shelf method to generate a normal map, which allows for an improved realism and increased details. \needcheck{need to be concrete?}

==> articles/copyright.tex <==
% \newpage
% \appendix


% We give the sources of images and mesh used in this paper (See Table~\ref{tab:copyright}). Other images not included in the table are either from the DTU dataset~\cite{aanaes2016large} or generated by Stable Diffusion~\cite{rombach2021highresolution}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}
  \centering
  \caption{Part 1/2 of Copyright Information}
    \small
    \resizebox{.85\textwidth}{!}{
    \begin{tabular}{c|c|c}
    \toprule
    Image/Mesh & Source & License \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/bag1.png}} & \multirow{2}{*}{https://pixabay.com/photos/leather-bags-duffel-bags-4379625/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/bag3.png}} & \multirow{2}{*}{https://pixabay.com/photos/mens-leather-bag-8073910/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/cat1.png}} & \multirow{2}{*}{https://pixabay.com/photos/cat-kitten-pets-animals-housecat-2934720/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/clock1.png}} & \multirow{2}{*}{https://pixabay.com/photos/clock-alarm-clock-time-time-display-2545142/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/frog3.png}} & \multirow{2}{*}{https://pixabay.com/photos/time-to-go-frog-farewell-travel-937265/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/horse.png}} & \multirow{2}{*}{https://pixabay.com/illustrations/mushroom-house-fantasy-cottage-4000133/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/house.png}} & \multirow{2}{*}{https://pixabay.com/illustrations/mushroom-house-fantasy-cottage-4000133/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/icecream1.png}} & \multirow{2}{*}{https://pixabay.com/photos/soft-ice-cream-soft-ice-cream-cone-50845/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/mushroom4.png}} & \multirow{2}{*}{https://pixabay.com/illustrations/toadstool-mushrooms-fantasy-1722288/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/rose.png}} & \multirow{2}{*}{https://pixabay.com/photos/rose-flower-petals-red-rose-320868/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/dinosaur2.png}} & \multirow{2}{*}{https://pixabay.com/illustrations/raptor-3d-model-render-dinosaur-5749823/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/teddy2.png}} & \multirow{2}{*}{https://pixabay.com/illustrations/teddy-bear-toy-stuffed-toy-teddy-7777659/} & \multirow{2}{*}{free to use} \\
    % & & \\
    % \midrule
    % \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/teddy.png}} & \multirow{2}{*}{Generated by Stable Diffusion} & \multirow{2}{*}{Apache License} \\
    % & & \\
    % \midrule
    % \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/napoleon.png}} & \multirow{2}{*}{ModelNet40~\cite{wu20153d}} & \multirow{2}{*}{academic research only} \\
    % & & \\
    % \midrule
    % \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/mushroom.png}} & \multirow{2}{*}{https://www.etsy.com/hk-en/listing/1214747045/red-mushroom-statue-colorful-painted-art} & \multirow{2}{*}{Fig~\ref{fig:mushroom_license}} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/rhino.png}} & \multirow{2}{*}{https://pixabay.com/photos/animal-wild-animal-rhino-africa-2765319/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/white_robot.png}} & \multirow{2}{*}{https://pixabay.com/illustrations/robot-humanoid-robot-machine-6654032/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/frog9.jpg}} & \multirow{2}{*}{https://pixabay.com/photos/frog-frog-prince-crown-figure-cute-1591901/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/bird_1.jpg}} & \multirow{2}{*}{https://pixabay.com/photos/one-leg-birds-nature-wildlife-beak-3393491/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/bird_7.jpg}} & \multirow{2}{*}{https://pixabay.com/photos/kingfisher-bird-perched-1867936/} & \multirow{2}{*}{free to use} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/bird2.jpg}} & \multirow{2}{*}{https://pixabay.com/illustrations/ai-generated-bird-rock-foliage-7976939/} & \multirow{2}{*}{free to use} \\
    & & \\
    % \midrule
    % \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/sculpture1.png}} & \multirow{2}{*}{https://www.pexels.com/photo/bust-of-septimius-severus-13865689/} & \multirow{2}{*}{free to use} \\
    % & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/mid_panda_2.png}} & \multirow{2}{*}{We generated it on Midjourney as a paid member in accordance with their agreement.} & \multirow{2}{*}{We own the asset.} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/mid_green_dog_1.png}} & \multirow{2}{*}{We generated it on Midjourney as a paid member in accordance with their agreement.} & \multirow{2}{*}{We own the asset.} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/mid_yellow_rabbit_3.png}} & \multirow{2}{*}{We generated it on Midjourney as a paid member in accordance with their agreement.} & \multirow{2}{*}{We own the asset.} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/mid_pink_robot2_2.png}} & \multirow{2}{*}{We generated it on Midjourney as a paid member in accordance with their agreement.} & \multirow{2}{*}{We own the asset.} \\
    & & \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:copyright1}%
\end{table*}%

\begin{table*}
  \centering
  \caption{Part 2/2 of Copyright Information}
    \small
    \resizebox{.85\textwidth}{!}{
    \begin{tabular}{c|c|c}
    \toprule
    Image/Mesh & Source & License \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/mid_whitebear_1_rgba.png}} & \multirow{2}{*}{We generated it on Midjourney as a paid member in accordance with their agreement.} & \multirow{2}{*}{We own the asset.} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/dog3_mids_1.png}} & \multirow{2}{*}{We generated it on Midjourney as a paid member in accordance with their agreement.} & \multirow{2}{*}{We own the asset.} \\
    & & \\
    \midrule
    \multirow{2}{*}{\includegraphics[height=0.7cm]{figures/img_copyright/mouse2_mids_2.png}} & \multirow{2}{*}{We generated it on Midjourney as a paid member in accordance with their agreement.} & \multirow{2}{*}{We own the asset.} \\
    & & \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:copyright2}%
\end{table*}%
% \begin{figure}
%     \centering
%     \includegraphics[width=0.25\textwidth]{figures/img_copyright/mushroom_license.png}
%     \caption{Copyright for Mushroom.}
%     \label{fig:mushroom_license}
% \end{figure}

% \begin{table*}[t]
% 	\begin{center}
%             % \tablestyle{2pt}{1.5}
% \begin{tabular}{c|c|c|l}
%             \toprule
%              Name & Image & Type & Description \\
%             \midrule
%             \multirow{2}{*}{\makecell{African \\ elephant}} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & an elephant native to Africa having enormous flapping ears and ivory tusks \\
%             & & chatgpt & massive, grey mammal with a long trunk, large ears, curved tusks, and wrinkled skin \\ 
%             \midrule
%             \multirow{2}{*}{charolais} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & this breed of cattle is heavy, with weighing 700-1650 kg. they have white/cream coats and pink noses \\
%             & & chatgpt & large, white-colored breed of cattle with a muscular build, broad forehead, and short horns \\ 
%             \midrule
%             \multirow{2}{*}{\makecell{Grevy's \\ zebra}} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & it resembles a mule with a big head, elongated nostril openings, large round conical ears, and tall erect mane \\
%             & & chatgpt & large, wild equid with black and white stripes, a white belly, and a tall, erect mane \\ 
%             \midrule
%             \multirow{2}{*}{box turtle} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & it has a domed shell hinged at the bottom, allowing them to close it tightly and escape predators \\
%             & & chatgpt & small, domed shell with brown or olive-colored skin and a pattern of yellow or orange spots or lines \\ 
%             \midrule
%             \multirow{2}{*}{tuatara} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & a reptile with a greenish-grey lizard-like appearance found only on certain small islands near New Zealand \\
%             & & chatgpt & a reptile with a spiny crest, two rows of teeth, and a third "eye" on the top of its head \\ 
%             \midrule
%             \multirow{2}{*}{\makecell{northern \\ seahorse}} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & northern seahorses have long snouts and a curly tail, and can grow up to 8 inches in length \\
%             & & chatgpt & the northern seahorse has a small body covered in bony plates, a long snout, and a curled tail \\ 
%             \midrule
%             \multirow{2}{*}{\makecell{lowland \\ burrowing \\ treefrog}} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & terrestrial burrowing nocturnal frog of grassy terrain and scrub forests having very hard upper surface of head \\
%             & & chatgpt & small, round-bodied frog with smooth skin, adapted for burrowing with short legs and a pointed snout \\ 
%             \midrule
%             \multirow{2}{*}{rock beauty} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & 
%             %gold and black butterflyfish found from West Indies to Brazil \\
%             predominately black. The head and front half portion of the body, and the caudal fin are a bright yellow \\
%             & & chatgpt & 
%             % the rock beauty has a yellow-orange body with black and blue accents on its fins, and a dark spot on its head \\ 
%             bright yellow head, tail, pectoral fins; black body, dorsal, anal fins; abrupt color transitions \\
%             \midrule
%             \multirow{2}{*}{clingfish} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & very small (to 3 inches) flattened marine fish with a sucking disc on the abdomen for clinging to rocks etc \\
%             & & chatgpt & the clingfish has a flattened body with a suction cup-like pelvic disc, and ranges in color from brown to green \\ 
%             \midrule
%             \multirow{2}{*}{porpoise} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & 
%             %any of several small gregarious cetacean mammals having a blunt snout and many teeth \\
%             whales distinguishable from dolphins by their more compact build, smaller size, and curved blunt snout with spatulate teeth \\
%             & & chatgpt & small, grey marine mammal with a rounded head, a small dorsal fin, and a curved mouth \\ 
%             \midrule
%             \multirow{2}{*}{manta} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & extremely large pelagic tropical ray with triangular pectoral fins, horn-shaped cephalic fins and large, forward-facing mouths \\
%             & & chatgpt & large, flat-bodied, wing-like fins, no tail, black or dark upper side, white or light underside \\ 
%             \midrule
%             \multirow{2}{*}{\makecell{aglais}} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & the wings of aglais are rusty red with a unique eyespot in black, blue, and yellow at each wingtip \\
%             & & chatgpt & eyespots on wings, blue-green-brown hues (European peacock butterfly) \\ 
%             \midrule
%             \multirow{2}{*}{\makecell{woodland \\ sunflower}} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & a wildflower native to the United States, which has bright yellow petals that surround a dark brown center \\
%             & & chatgpt & tall yellow flower with numerous thin petals surrounding a dark center disk, and green leaves \\ 
%             \midrule
%             \multirow{2}{*}{calliandra} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & the flowers are produced in cylindrical or globose inflorescences and have numerous long slender stamens \\
%             & & chatgpt & small shrub with fern-like leaves and vibrant, pink, powder-puff shaped flowers \\ 
%             \midrule
%             \multirow{2}{*}{\makecell{cistus \\ salviifolius}} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & a shrub with fragrant, silver-green foliage and white flowers \\
%             & & chatgpt & a tall, bright yellow or orange flower often grown for its edible seeds and as an ornamental plant \\ 
%             \midrule
%             \multirow{2}{*}{\makecell{power drill}} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & 
%             %a power tool for drilling holes into hard materials \\
%             a hand tool with a rotating chuck driven by an electric motor for drilling \\
%             & & chatgpt & handheld tool with a motor and rotating chuck for drilling holes and fastening screws, often with a pistol grip \\ 
%             \midrule
%             \multirow{2}{*}{clarinet} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & 
%             %a single-reed instrument with a straight tube \\
%             the clarinet is a single-reed instrument with a nearly cylindrical bore and a flared bell. \\
%             & & chatgpt & narrow, cylindrical woodwind instrument with a mouthpiece, reed, and numerous keys for playing different notes \\ 
%             \midrule
%             \multirow{2}{*}{\makecell{off-road \\ vehicle}} & \multirow{2}{*}{\includegraphics[height=1cm]{figures/albedo_reg.pdf}} & Experts & the off-road vehicles typically have four-wheel-drive, increased suspension, and large tires \\
%             & & chatgpt & large, sturdy vehicle with high ground clearance, wide tires, and typically four-wheel drive for use on unpaved terrain \\ 
%             \bottomrule
%             \end{tabular}
% 	\end{center}
%         \vspace{-15pt}
%  	\caption{
% 		Examples of category descriptions of V3Det.
% 	}\label{tab:description}
% 	\vspace{-10pt}
% \end{table*}

==> tables/dtu_geometry.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \caption{\textbf{Geometry evaluation on the DTU dataset.} $CD_{full}$ denotes the standard Chamfer Distance; $CD_{partial}$ quantifies the distance from the partial ground truth to the complete 3D output only.}
    \small
    \resizebox{.48\textwidth}{!} {
    \begin{tabular}{l|ccccc}
    \toprule
    
    Method & \multicolumn{1}{l}{Shap-E} & \multicolumn{1}{l}{Neurallift-360} & \multicolumn{1}{l}{Realfusion} & \multicolumn{1}{l}{Zero-1-to-3} & \multicolumn{1}{l}{Ours} \\
    \midrule
    $CD_{full} \downarrow$ & 0.039 & 0.045 & 0.037 & 0.038 & \textbf{0.035} \\
    $CD_{partial} \downarrow$ & 0.036 & 0.042 & \textbf{0.032} & 0.036 & \textbf{0.032} \\
    \bottomrule
    
    \end{tabular}%
    }
  \label{tab:dtu_geo}%
\end{table}%

